Private, Anonymous, Collateralizable Commitments vs. MEV

In this work, we introduce the private, anonymous, collateralizable commitments (PACCs) framework. PACCs allow any smart contract wallet holder to collateralize a claim, request, or commitment in general, in a private and anonymous manner. PACCs can prove arbitrarily much or little about the wallet generating the commitment, and/or the transaction which is being committed. We demonstrate that PACCs can be applied to effectively eliminate maximal-extractable value (MEV) in DeFi where it currently occurs, shifting MEV instead to censorship. After describing our protocol with detail, we provide an implementation using the Ethereum blockchain, and whose benchmarks prove how PACCs are completely feasible.

==> notes/JamesNotes.tex <==
\section{Chat with James}

\subsection*{Questions/Thoughts}

\begin{itemize}
    \item Is there spam protection?
    \item How do orders get executed?
\end{itemize}

James is looking at differential privacy for trading protocols. Basically adding fuzzy liquidity to a DEX protocol. 

==> sections/EthResearch.tex <==
This post provides a high-level overview of DPACCs, a commitment scheme which can be built on top of existing smart contract wallet (SCW) architecture. DPACCs allow any SCW holder to collateralize an on-chain commitment in a private and anonymous manner. DPACCs can prove arbitrarily much or little about the wallet generating the commitment, and/or the transaction which is being committed. This can be used to convince a prospective block builder or relayer that the wallet generating the DPACC has enough funds to pay required fees, that the wallet is committed to performing certain actions, and importantly, that the wallet loses some amount of collateral if this commitment is broken. DPACCs delegate typically expensive zero knowledge operations off-chain, only requiring an additional one or two mapping checks when compared to transactions being sent from basic externally owned accounts.

**ZK Primer** For this article, we need a function that allows us to prove set-membership in zero knowledge. In the following $h()$ is a hash function, and $||$ is string concatenation. We define that function as follows. For a set of commitments $\textit{Commits}$, NIZKPoK($\mathcal{S},\mathcal{R},\textit{Commits}$) returns a string $\mathcal{S}$ and non-interactive proof of knowledge that the person running \textit{NIZKPoK}() knows an $\mathcal{R}$ such that the commitment $h(\mathcal{S} || \mathcal{R}) $ is in $ \textit{Commits}$. Importantly, 
\begin{enumerate}
    \item $\mathcal{R}$ is not revealed, so the verifier of the proof does not learn which commitment in $\textit{Commits}$ the proof corresponds to.
    \item This revelation identifies to a verifier when a proof has previously been provided for a particular, albeit unknown, commitment as the prover must reproduce $\mathcal{S}$.
\end{enumerate}

There are many tools to achieve this, including those used in Tornado Cash, Semaphore, ZCash, and others.


\subsubsection{DPACCs}

It suffices to consider SCWs as extensions of externally-owned accounts on which we can apply additional constraints. For $W$ the set of all wallets, and some wallet $w \in W$, $w$ can be considered as a set of tokens. To reason about DPACCs, we need two mappings.
\begin{itemize}
    \item For every SCW $w$, a \textit{secret commitment mapping} $C^w_S: \{0,1\}^{\Theta(\kappa)} \rightarrow B \subseteq w$. $C^w_S(x)$ is such that if $x \neq y$, $C^w_S(x) \cap C^w_S(y) = \emptyset$.
    \item A \textit{global transaction commitment mapping} $C_T: \{0,1\}^{\Theta(\kappa)} \rightarrow \{0,1\}^{\Theta(\kappa)}$.
\end{itemize}

Players in our system using SCWs maintain a mapping of secret commitments to tokens within their wallet. To use tokens in a wallet, users must provide a signed transaction, as in a basic externally-owned account, and the secret corresponding to a commitment/commitments within the wallet. Revealing the secret $\mathcal{S}$ corresponding to a non-zero commitment $\textit{com}=h(\mathcal{S}||\mathcal{R})$ forces $w$ to use only tokens in $C^w_S(\textit{com})$. At the end of a transaction, the user must generate new mappings for all unmapped tokens in the SCWs, with the default being the 0-secret commitment. If $C^w_S(\textit{com}=h(\mathcal{S}||\mathcal{R}))=X$ for some set of tokens $X$, $X$ is fixed (tokens cannot be added or removed from $X$) until $\mathcal{S}$ is revealed.

A further restriction on SCWs is the verification that a revealed secret corresponds to a valid entry in the global transaction commitment mapping. At initialization, $C_T(x)=0, \ \forall x \in \{0,1\}^{\Theta(\kappa)}$. When a SCW $w$ signs a transaction $tx$ and attempts to use tokens $X\subseteq C^w_S(\mathcal{S})$, it must be that either  $C_T(\mathcal{S}) = 0 $, or $C_T(\mathcal{S}) = h(tx)$.
Otherwise, the transaction is aborted. To add a mapping $C_T: x \rightarrow y$, we require that $C_T(x)=0$ and $y$ is provably signed by the player who generated $x$ using some pre-defined PKI. 

**Example of how DPACCs can thwart MEV**

Consider a set of wallets $\{w_1,...,w_n\}=W$ with non-zero secret commitment mappings to their token balances. That is, any wallets in $W$ must reveal the committed secret in order to use their tokens balances. SCWs integrated to use DPACCs can transact as normal, revealing the commitment secret corresponding to tokens, and then using these tokens for normal transactions, as is done with externally owned accounts. This requires first verifying the mapping in the SCW, then verifying that the secret does not correspond to a mapping in the global transaction commitment mapping. Two mapping checks are cheap (much less than 20k gas, the cost for inserting to mapping, although not sure exactly).

DPACCs become interesting when one of the SCWs wants to insert a DPACC into the global transaction commitment mapping.
Auctions demonstrate the power of DPACCs. Consider an auction occurring where buyers and sellers are allowed to join until a fixed cut-off. Revealing order information before all players have committed to their orders is an elementary source of MEV. Instead of sending plain-text transactions, users can send DPACCs. 

Let's say a user $u_i$ wanting to sell 1 ETH for USDC creates a sell order for 1 ETH. The user generates a commitment for the transaction $tx=\textbf{pay fee to relayer}|| \textbf{sell 1 ETH for USDC}$. 

The users generates two proofs to be sent with $h(tx)$ to a relayer pool:
\begin{enumerate}
    \item NIZKPoK($\textbf{pay fee to relayer}, \textbf{sell 1 ETH for USDC},\{h(tx)\}$). Recalling the primer on ZK subsection, this proves that the prefix of the transaction committed by $h(tx)$, which the relayer can see, pays a relayer a fee if it is included in the blockchain, but doesn't reveal anything about the rest of $tx$.
    \item NIZKPoK($\mathcal{S}, \mathcal{R},\textit{Commits}$), for $\textit{Commits}$ being the set of secret commitments of wallets with balances of at least $0.1$ ETH or $100$ USDC, after fees. Any relayer with access to the chain state can verify if this proof is correct. Specifically, the verifier knows that if $\mathcal{S} \rightarrow h(tx)$ is added to the global transaction commitment mapping, $u_i$ must reveal $tx$, or lose at least  $0.1$ ETH or $100$ USDC if the transaction is not revealed. In reality, the user in question loses at least $1$ ETH, but this is not important to the relayer.
\end{enumerate}

If $h(tx)$ is added to the transaction commitment mapping, $u_i$ must reveal $tx$. This is because $u_i$ must reveal $\mathcal{S}$ to use the tokens in her wallet. As $\mathcal{S}$ maps to $h(tx)$, the only valid transaction that can be executed is $tx$. Therefore, if the auction contract punishes late revelation, as $u_i$ committed to an order in the auction, $u_i$ is effectively forced to reveal this order. If all orders must be committed before the revelation phase, the entire auction consists of committed orders which reveal nothing consequential about the orders, or the players who committed to them. 

As such, DPACCs allow integrated SCW users to join any ongoing auction, whether it be a DEX auction (see batch auctions and their price guarantees under competition \cite{FrequentBatchAuctionsBudish}), NFT auction, or liquidation auction, all \textbf{without} being subjected to MEV. 



==> sections/Proofs.tex <==



\begingroup
\def\thetheorem{\ref{lem:diminishingCol}}
\begin{lemma}
    For a base PACC transaction $tx$ from a wallet $w$ with $bal(w)>fee$, the Nash Equilibrium for $collateral=0$.
\end{lemma}
\endgroup

\begin{proof} 
    For any wallet $w$ posting a commitment to such a transaction $tx$ with $bal(w)>fee$, the payoff for revealing $tx$ is at least $collateral$, compared to $0$ for not revealing. Therefore, any collateral greater than 0 is sufficient to incentivize revelation. Given a cost to $w$ for locking collateral, the optimal collateral for $w$ is 0. Therefore, $w$ posts the minimum possible collateral, which approaches 0. 
\end{proof}


\begingroup
\def\thetheorem{\ref{lem:PACCAuctions}}
\begin{lemma}
    Sealed-bid auctions can be run on-chain among all wallets $W$ such that $bal(w)>fee, \ \forall \ w \in W$. 
\end{lemma}
\endgroup

\begin{proof} 
    Consider such a wallet $w \in W$, and an on-chain auction $A$. Let $A$ accept bid commitments for $\revealTXDelay$ blocks, followed by $\revealTXDelay$ blocks in which bids committed to $A$ can be revealed.
    Consider a base PACC transaction $tx$, with $tx_2 \equiv \textit{bid X in auction }A$ for some set of tokens $X$. We know for any $w \in W$ committing to $tx$ and proving membership in $W$, a relayer adds $\commit(tx)$ to the blockchain within $\revealTXDelay$ blocks. Therefore any $w \in W$ submitting this bid commitment and proofs to a relayer is included in $A$. Put differently, after the initial $\revealTXDelay$ blocks, any player who wanted to commit a bid for $A$ has been included in the blockchain. 
    
    After the initial $\revealTXDelay$ blocks, all players reveal their bids. As bids can be revealed for up to $\revealTXDelay$ blocks, this is sufficiently long for all players revealing bids to be added to the blockchain. As the committed transactions are base PACC transactions, all players committing to a bid are incentivized to reveal. Importantly, all bids were committed before any information regarding other bidders was revealed, with revealed bids matching committed bids due to the requirement of the global transaction commitment mapping for revealed transactions from $w$ to match any transaction committed by $w$.
    
    Thus, at the end of $\revealTXDelay$ blocks, all bids are revealed on chain. Any player in the blockchain can then settle the auction, deducing the auction winner and settlement price from the revealed bids. This is sufficient to run a sealed-bid auction. 
\end{proof}

\begingroup
\def\thetheorem{\ref{cor:PACCFBAs}}
\begin{corollary}
  Frequent batch auctions can be run on-chain among all wallets $W$ such that $bal(w)>fee, \ \forall \ w \in W$. 
\end{corollary}
\endgroup



\begin{proof} 
   From Lemma \ref{lem:PACCAuctions}, we know we can implement any auction involving sealed-bids in any set of tokens. For any pair of token sets $(X,Y)$, consider an auction $A$ where players submit bids as base PACC transactions, of the form $tx_1||tx_2$, with $tx_2$ equivalent to \textit{buy $v_x>0$ of $X$ for $v_y>0$ of $Y$} or \textit{buy $v_y>0$ of $Y$ for $v_x>0$ of $X$}. If the auction is run over $2\revealTXDelay$ blocks, this is enough for players to commit sealed bids to the blockchain, and have them revealed. From \cite{FairTraDEXMcMenamin}, we can implement an on-chain clearing-price verifier to ensure orders of this format get executed at a unique clearing price which maximizes traded volume, and as such, replicates a frequent batch auction. 
\end{proof}


\begingroup
\def\thetheorem{\ref{sec:RFQ}}
\begin{lemma}
    Given no transaction fees, the PACC RFQ protocol has Nash Equilibrium involving MMs committing user orders to the blockchain with $E(f_H)=0$.
\end{lemma}
\endgroup

\begin{proof}
   Firstly, given the order is generated when the external market price is $\MIFP$, for any block generated after this point (after block $H$), the expected external market price is $\MIFP$ due to the Martingale assumption. As all MMs observe $\MIFP$, the expected revenue for a MM responding to a PACC RFQ is at least 0 and strictly increasing in block height, making this a Dutch Auction in the commission specified by $f_H()$ between MMs. By the revenue equivalence principle \cite{krishna2009auction}, the expected revenue for the seller is the same as if this were an sealed-bid auction to receive $f_H()$. For any positive value of $f_H$, MMs will bid for this opportunity. As the user chooses $f_H()$, the commission to pay, but does not receive the revenue of the auction, for any positive value for $f_H(h)$, $h \geq H$, the user is strictly incentivized to reduce $f_H(h)$. As such, $E(f_H)=0$. 
\end{proof}
